Generation and Manipulation of Entanglement in Quantum Optical Systems

In this thesis, several new procedures for the generation and manipulation of entangled states in quantum optical systems are introduced. Each is evaluated in terms of realistic models of the imperfect apparatus of any real laboratory implementation. The first half of the thesis considers entanglement generation in Cavity QED, introducing several proposals for the creation of maximally entangled two-qubit states. The second half of the thesis focuses on the manipulation of entangled states of light pulses. In particular, an entanglement distillation procedure for Gaussian states is introduced. This combines a Procrustean protocol for the generation of highly entangled non-Gaussian states, with a "Gaussification" procedure, which allows more highly entangled approximately Gaussian states to be distilled from a non-Gaussian supply.

==> abstract.tex <==
%auto-ignore
In this thesis, we introduce and evaluate several new procedures for the generation and manipulation of entangled states in quantum optical systems. Each scheme is evaluated in terms of realistic models of the imperfect apparatus of any real laboratory implementation. 

The first set of proposals concern atoms interacting with optical cavities.
We describe a novel method of generating maximally entangled states in the states of the electromagnetic fields of two microwave cavities mediated by the passage of an atom between them and its subsequent measurement. We show that this approach has a natural robustness against a variety of experimental imperfections. 

We then introduce a further scheme for the generation of maximally entangled states between pairs atoms or ions trapped in spatially separate cavities. The scheme proceeds by the weak driving of a transition in each ion. Photons leaking from the cavities are mixed on a beam splitter before reaching detectors, so that which-path information about the photon's source is erased. The detection heralds the creation of a maximally entangled state between the atoms. In the ideal case, this leads to the deterministic generation of high fidelity states, and when more realistic conditions are assumed, still allows high fidelity states to be generated in a heralded non-deterministic manner.

In the final part of the thesis, we turn our attention to the manipulation of entangled states of light pulses. Entanglement distillation, the ability produce a small number of highly entangled separated systems from a large supply of weakly entangled systems, has many applications in quantum information science. Gaussian states are the natural states of light pulses produced in laser experiments, and  standard optical operations preserve this form.
Recent results have shown that it is impossible to implement entanglement distillation on Gaussian states with these standard optics alone. We illustrate that the additional element of photon detection enables one to circumvent this restriction, but produces highly non-Gaussian states. Highly entangled Gaussian states have many applications in quantum information science. We introduce a simple  protocol, which we call Gaussification, which allows more highly entangled approximately Gaussian states to be distilled from a non-Gaussian supply. Together, these procedures form the first realistic entanglement distillation scheme for Gaussian states. We analyse fully the convergence characteristics the protocol and assess the operation of the scheme with the imperfect operations one could expect in a real laboratory implementation.
%%% Local Variables: 
%%% mode: plain-tex
%%% TeX-master: "C:\\Documents and Settings\\dan\\My Documents\\Thesis\\Chapters\\thesis"
%%% End: 


==> c-8b.tex <==
%auto-ignore
\chapter{``Gaussification'' with Linear Optics}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Introduction}

In this section we introduce an iterative protocol, which we shall call ``Gaussification'' \cite{brownegauss,jensgauss}. This protocol acts on a supply of  many copies of a non-Gaussian two-mode entangled state, under  conditions which we describe below. It then, after several non-deterministic iterations produces a small number of states which are arbitrarily close to Gaussian states and which, furthermore, are often more entangled than their input. %Pure input states lead to pure output and for mixed input states, the output state can be of lower entropy and even, under certain circumstances pure.
First we will outline the protocol and then, under the assumption that all operations are ideal we will consider analytically all its important properties. In the following chapter we will then model how the procedure would be affected by the most important experimental imperfections of a real implementation of the scheme.




\begin{figure}
\includegraphics[width=14cm]{gausprot}
\caption{\label{gausfig}A single iteration of the ``Gaussification'' protocol.  }
\end{figure}



 Each step of the protocol proceeds as illustrated in figure~\ref{gausfig}. It is an iterative procedure. Each iteration consists of
\begin{enumerate}
\item In the first instance, Alice and Bob act on shared two-mode entangled states supplied from a source. In later iterations they use pairs of states generated by a previous successful iteration.
\item The each mix their half of two copies of the state on a 50:50 beam splitter.
\item They measure one of the outputs with a detector which  distinguishes the presence from the absence of photons.
\item If no photons are registered, the iteration was a success, and the resultant state is saved for the next iteration.
\end{enumerate}


Before we investigate the properties  of this protocol for  arbitrary input states, let us illustrate it using the simple input state $\ket{\psi^{(0)}}=\ket{00}+\eta\ket{11}$. We label the two entangled modes 1 and 2 and use the labels $A$ and $B$ to denote Alice and Bob. Thus the initial state of the two copies of $\ket{\psi^{(0)}}$ is

\begin{equation}\begin{split}
\ket{\psi^{(0)}}\otimes\ket{\psi^{(0)}}=&\ket{0}_{A1}\ket{0}_{B1}\ket{0}_{A2}\ket{0}_{B2}+\eta \ket{1}_{A1}\ket{1}_{B1}\ket{0}_{A2}\ket{0}_{B2}\\&\mbox{}+\eta\ket{0}_{A1}\ket{0}_{B1}\ket{1}_{A2}\ket{1}_{B2}+\eta^2\ket{1}_{A1}\ket{1}_{B1}\ket{1}_{A2}\ket{1}_{B2}\ .
\end{split}
\end{equation}
The 50:50 beam-splitter transformation transforms the state,
%
\begin{equation}\begin{split}
\ket{\psi^{(0)}}\rightarrow&\ket{0}_{A1}\ket{0}_{A2}\ket{0}_{B1}\ket{0}_{B2}+\frac{\eta}{2} \bigl(\ket{1}_{A1}\ket{0}_{A2}+\ket{0}_{A1}\ket{1}_{A2}\bigr)\bigl(\ket{1}_{B1}\ket{0}_{B2}+\ket{0}_{B1}\ket{1}_{B2}\bigr)\\&\mbox{}+\frac{\eta}{2} \bigl(-\ket{1}_{A1}\ket{0}_{A2}+\ket{0}_{A1}\ket{1}_{A2}\bigr)\bigl(-\ket{1}_{B1}\ket{0}_{B2}+\ket{0}_{B1}\ket{1}_{B2}\bigr)\\&\qquad\mbox{}+\frac{\eta^2}{2} \bigl(-\ket{2}_{A1}\ket{0}_{A2}+\ket{0}_{A1}\ket{2}_{A2}\bigr)\bigl(-\ket{2}_{B1}\ket{0}_{B2}+\ket{0}_{B1}\ket{2}_{B2}\bigr)
\end{split}
\end{equation}
so that, conditional on a measurement of zero photons in modes $A2$ and $B2$, the state is transformed to

\begin{equation}
\ket{\psi^{(1)}}=\ket{0}_{A1}\ket{0}_{B1}+\eta\ket{1}_{A1}\ket{1}_{B1}+\frac{\eta^2}{2}\ket{2}_{A1}\ket{2}_{B1}\ .
\end{equation}
The probability of obtaining these measurement outcomes is $(1+\eta^2+\eta^4/4)/(1+\eta^2)^2$, which for $\eta=0.5$ is approximately  0.8. We observe that the state remains a superposition of states of equal photon number and also that the ratio between the coefficients of $\ket{00}$ and $\ket{11}$ has remained constant. It is simple to calculate the state produced after a further iteration. In figures~\ref{fig:pureentt} and~\ref{fig:pureprob} we plot the entanglement of the state produced after the 1st and 2nd iterations, and the success probability each time. We see, that for all values of $\eta$, each iteration generates a state with a higher degree of entanglement. Furthermore, the success probability for each iteration for all values of $\eta$ is high, staying between 25\% and 100\%.


\begin{figure}
\psfrag{en}{\large $E_\mathcal{N}$}
\psfrag{lam}{\large $\eta$}
\begin{center}
\includegraphics{pureent.eps}
\end{center}
\caption{\label{fig:pureentt}This figure depicts the logarithmic negativity $E_\mathcal{N}$ as a function of $\eta$ for, i) the state $\ket{\psi}=\sqrt{1/(1+\eta^2)}(|0,0\rangle+\eta|1,1\rangle)$ used as input supply for the Gaussification (dotted line), ii) the state generated by a single (dashed) and two iterations (wider dashing) of the protocol and iii) the limiting two-mode squeezed state which, in the ideal case, will be reached after many iterations.
We use the logarithmic negativity here for ease of comparison with the mixed state cases later in the chapter. }
\end{figure}
\begin{figure}
\psfrag{pr}{\large $P$}
\psfrag{lam}{\large $\eta$}
\begin{center}
\includegraphics{pureprob.eps}
\end{center}
\caption{\label{fig:pureprob} Here we see the success probability $P$ for the first (dashed) and second (wider dashing) iterations of the protocol with input supply $\ket{\psi}=\sqrt{1/(1+\eta^2)}(|0,0\rangle+\eta|1,1\rangle)$.}
\end{figure}





To see if these features apply to other input states, we now consider inputs of the more  general form $\ket{\psi^{(0)}}=\sum_n \alpha_n^{(0)} \ket{n,n}$. States generated by successful iterations retain this form. Let us   introduce the notation $\ket{\psi^{(i)}}=\sum_n \alpha_n^{(i)} \ket{n,n}$ for the state generated after $i$ successful iterations of the Gaussifier. By writing out the action of the beam-splitter and measurement on this general state one finds a recurrence relation relating the coefficients of the $(i+1)$th states to the $i$th,

\begin{equation}
\label{eq:recursion}
    \alpha_{n}^{(i+1)}= 2^{-n}\sum_{r=0}^{n} {n \choose r}
    \alpha_{r}^{(i)} \alpha_{n-r}^{(i)} \ .
\end{equation}

This relation allows us to investigate the effect of many iterations of the protocol. First, we can ask which states remain unchanged by the scheme. Let us label such a state $\ket{\psi}^{(\infty)}$ and its coefficients  $\alpha_{n}^{(\infty)}$. These must be solutions to the equations
\begin{equation}\label{eq:fixedschmidt}
    \alpha_{n}^{\infty}= 2^{-n}\sum_{r=0}^{n} {n \choose r}
    \alpha_{r}^{(\infty)} \alpha_{n-r}^{(\infty)} \ .
\end{equation}
for all $n$. We solve these equations  inductively. The 0th equation gives us $\alpha_0^{(\infty)}=(\alpha_0^{(\infty)})^2$, therefore $\alpha_0^{(\infty)}=1$. Of course, since the states are not normalised, this alone does not specify the state at all. Setting $\alpha_0^{(\infty)}=1$, the $n=1$ equation gives us $\alpha_1^{(\infty)}=\alpha_1^{(\infty)}$. We therefore have a free choice for this parameter, and set it to $\zeta$. Proceeding we find that $\alpha_2^{(\infty)}=\zeta^2$ and  $\alpha_3^{(\infty)}=\zeta^3$, and this pattern continues. In fact the general solution to equations~\eqref{eq:fixedschmidt} is $\alpha_n^{(\infty)}=\zeta^n$, which can be verified immediately by substitution. This state is nothing other than the two-mode squeezed state with squeezing $\tanh(r)=-\zeta$.

Since this family of states are the only fixed points of the iteration, given a starting state in the form, $\ket{\psi^{(0)}}=\sum_n \alpha_n^{(0)} \ket{n,n}$ repeated iterations must, if they converge, lead, in the limit of many iterations, to a two-mode squeezed state, a Gaussian state. We can investigate the convergence via recurrence relations~\eqref{eq:recursion}. For convenience, let us adopt a normalisation convention where $\alpha^{(0)}_0=1$. As we have already seen, this means that $\alpha_0^{(i)}$ remains at this value. Similarly, in this normalisation convention $\alpha_1^{(i)}$ also remains at its initial value. We prove the convergence of the remaining coefficients by induction. We first postulate that each coefficient will converge to the value $\alpha_n^{(\infty)}$, and for that aim introduce deviations form this final value $\delta_n^{(i)}=\alpha_n^{(i)}-\alpha_n^{(\infty)}$. We can now rewrite equation~(\ref{eq:recursion})
\begin{equation}
\delta_n^{(i+1)}=2^{-n}\sum_{r=0}^n{n \choose r}\left( \delta_r^{(i)} \delta_{n-r}^{(i)}- \delta_r^{(i)}\alpha_{n-r}^{(\infty)}- \delta_{n-r}^{(i)}\alpha_{r}^{(\infty)}\right)
\end{equation}
Let us take the limit that $i$ goes to infinity and assume that all coefficients $\alpha_m^{(i)}$ for $m<n$ converge to $\alpha_m^{(\infty)}$ in this limit.

\begin{equation}
\lim_{i\to\infty}\left(\delta_{n}^{(i+1)}\right)=2^{(1-n)}\lim_{i\to\infty}\left(
\delta_{n}^{(i)}\right)
\end{equation}
Thus as long as $2^{1-n}<1$, that is as long as $n>1$, if all coefficients $\alpha_m^{(i)}$ converge to $\alpha_m^{(\infty)}$ for $m<n$,  $\alpha_m^{(i)}$ will converge to  $\alpha_m^{(\infty)}$ in the limit that $i$ tends to infinity. Since we have already shown that $\alpha_0^{(i)}$ and $\alpha_1^{(i)}$ converge, the convergence of the other coefficients follows by induction. This means that formal  convergence in the coefficients occurs for all input states. However not all these final states correspond to physical states. In particular, when $\zeta\ge1$, the state $\sum_n\zeta^n\ket{n,n}$ is unnormalisable, and therefore not a physical state. Thus we conclude the following, for an large input supply of states in the form $\ket{\psi^{(0)}}=\sum_n \alpha_n^{(0)} \ket{n,n}$, repeated iteration of successful runs of the Gaussification protocol lead to the generation of a small number of two-mode states with squeezing $\tanh(r)=-\alpha_1^{(i)}/\alpha_0^{(i)}$ as long as $\alpha_1^{(i)}/\alpha_0^{(i)}<1$, otherwise the procedure does not converge.


We can illustrate the way the state converges toward Gaussian form, by plotting the Wigner function of the single-mode states of the reduced
state of one mode alone for the initial state with parameter $\eta$ set to 0.6, and the state
after one and two steps.
The Wigner function %$W:{\mathbbm{R}}^{2}\longrightarrow
%{\mathbbm{R}}$ 
is the Fourier
transform of the characteristic function,
\begin{equation}
        W(\xi) = \frac{1}{(2\pi)^2} \int e^{i \xi^T \Sigma \eta} \chi(\eta) d^2 \eta.
\end{equation}
Figure~\ref{fig:Wigner} shows the Wigner function of the Bob's reduced state initially and after one and two iterations of the protocol. While initially, the Wigner function is
far from being a Gaussian in phase space, its non-Gaussian features
disappear quickly.

\begin{figure}[th]
\centerline{
\includegraphics[width=6.5cm]{WignerFunction1New.eps}
}
\centerline{
\includegraphics[width=6.5cm]{WignerFunction2New.eps}
}
\centerline{
\includegraphics[width=6.5cm]{WignerFunction3New.eps}
}

\vspace{.2cm}
\caption{\label{fig:Wigner} The Wigner function of the reduced
state of  one system initially and after one and two steps for the
initial pure state $\ket{\psi}\propto\ket{0,0}+0.6\ket{1,1}$.}
\end{figure}



\section{General Input States}\label{sec:geninput}

In the previous section we  illustrated the Gaussification procedure with  simple pure states as input. Now we turn consider input states which are completely general,  pure or mixed states $\rho^{(0)}$. We will proceed in the same line of  analysis which was applied in the previous section. We will thus prove, that
\begin{enumerate}
\item All two-mode Gaussian states with zero displacement vector are invariant under the Gaussification iteration
\item Beginning with an arbitrary input supply, the protocol will either lead to convergence to a particular Gaussian state or it will not converge.
\item Give analytic forms for the convergence and the limiting states for a given input $\rho^{(0)}$ in terms of its matrix elements.
\end{enumerate}

The proof that all two-mode Gaussian states are invariant can be achieved in a straight-forward manner, using the covariance matrix formalism. Let the covariance matrix of $\rho^{(0)}$ be $\Gamma$. The covariance matrix of Alice and Bob's pair of two-mode states will be $\Gamma\oplus\Gamma$, where the modes are ordered $A1$, $B1$, $A2$, $B2$. The symplectic 50:50 beam-splitter operation $S$ is
\begin{equation}
S=\sqrt{\frac{1}{2}}\left(\begin{array}{cc} \iden_2 & -\iden_2\\ \iden_2 & \iden_2
  \end{array}\right)
\end{equation}

Since the beam-splitter operation will be applied to modes in pairs $A1$, $A2$ and  $B1$, $B2$ (not the above order) we also need a swap operation $\Lambda$ 
%
\begin{equation}
\Lambda=\left(\begin{array}{cc} 0 & \iden_2\\ \iden_2 & 0
  \end{array}\right)
\end{equation}
%
Thus the application of beam-splitters to $\rho^{(0)}$ can be expressed
%
\begin{equation}\begin{split}
&\Gamma\oplus\Gamma \rightarrow(\iden_2\oplus\Lambda\oplus \iden_2)(S\oplus S)(\iden_2\oplus\Lambda\oplus \iden_2)\Gamma\oplus\Gamma(\iden_2\oplus\Lambda\oplus \iden_2)(S\oplus S)^T(\iden_2\oplus\Lambda\oplus \iden_2)\\&\qquad\qquad=\Gamma\oplus\Gamma\ .
\end{split}
\end{equation}
%
%
%
Thus the action of simultaneously mixing modes $A1$ and $A2$, and $B1$ and $B2$ leaves the covariance matrix of the states invariant. 

Now let us look at how displacement vector is transformed. Let $\vek{d}$ be the displacement vector of $\rho^{(0)}$. The beam-splitters transform $\vek{d}$ thus,
%
%
%
\begin{equation}
\vek{d}\oplus\vek{d} \rightarrow (\iden_2\oplus\Lambda\oplus \iden_2)(S\oplus S)(\iden_2\oplus\Lambda\oplus \iden_2)\vek{d}\oplus\vek{d}=\vekk{0}\oplus\sqrt{2}\vek{d}
\end{equation}
where $\vekk{0}$ is the zero vector.
%
Thus, after the measurement of modes $A2$ and $B2$, the resultant state is a Gaussian state with the same covariance matrix as $\rho^{(0)}$ and zero displacement vector. This proves the first of our assertions above.

To analyse the convergence properties of the protocol for a general input we proceed as above, constructing a recurrence relation for the matrix elements of the state $\rho^{(i)}$ produced after $i$ successful iterations.
where
\begin{equation}\label{recurrence1}
        \rho_{a,b;c,d}^{(i+1)} =
        \sum_{s=0}^a
        \sum_{t=0}^b
        \sum_{n=0}^c
        \sum_{m=0}^d
        M_{a,b;c,d}^{s,t;n,m} 
        \rho^{(i)}_{s,t;n,m} \rho_{a-s,b-t;c-n,d-m}^{(i)}\ .
\end{equation}
with coefficients $M_{a,b;c,d}^{s,t;n,m}$ given by
\begin{equation}\label{nl1}
        M_{a,b;c,d}^{s,t;n,m}  =
        2^{-(a+b +c+d)/2} (-1)^{(a+b+c+d)-(s+t+n+m)}
        \left[
        \binom{a}{s}
        \binom{b}{t}
        \binom{c}{n}
        \binom{d}{m}
        \right]^{1/2}\ .
\end{equation}
We first observe that all matrix elements $\rho_{a,b,c,d}^{(i)}$ where $(a+b+c+d)$ is odd will vanish after the first iteration, since the terms in the sum of equal amplitude pick up opposite signs and cancel out.
Following the notation which we used above, we label a state which is invariant under this map $\rho^{(\infty)}$. We find that either  $\rho^{(\infty)}_{0,0,0,0}=1$ or $\rho^{(\infty)}_{0,0,0,0}=0$. In this latter case, all other matrix elements are also zero, so we ignore this trivial non physical case.  If we  normalise the state such that $\rho^{(\infty)}_{0,0,0,0}=1$, the following six coefficients of $\rho^{(\infty)}$ are completely free; $\rho_{1,0,1,0}^{(\infty)}$,  $\rho_{0,1,0,1}^{(\infty)}$, $\rho_{1,0,0,1}^{(\infty)}$, $\rho_{2,0,0,0}^{(\infty)}$, $\rho_{1,1,0,0}^{(\infty)}$. One can then show by induction that once these 10 parameters (since two of the elements are real) are chosen, all other matrix elements are already determined. In fact $\rho_{a,b,c,d}$ is a polynomial in these elements of degree $D\le \textrm{Max}\{a,b,c,d\}$.

We now need to show that all of these fixed points correspond, if they correspond to physical states, to zero-displacement Gaussian states whose covariance matrices are uniquely specified by these 10 parameters.
To do this, we calculate the relevant matrix elements for a general zero-displacement Gaussian state. We start with equation~(\ref{gausstaterho}), substituting the relevant characteristic function,

\begin{equation}
\rho=\frac{1}{(2\pi)^2}\int\exp[-\frac{1}{4} \vekk{\xi}^T\Sigma \Gamma \Sigma^T \vekk{\xi}]
\hat{W}_\vekk{\xi}
d^{2n}\xi \ .
\end{equation}
The matrix elements of the Weyl operator can be calculated via it's normal ordered form \cite{cahillglauber}. This gives the following,
\begin{equation}
\begin{split}
&\langle m|W(\vekk{\xi})|n\rangle=\\&\left(\frac{n!}{m!}\right)^{\frac{1}{2}}e^{-\frac{(\xi_1^2+\xi_2^2)}{4}}\left(\frac{\xi_1+i\xi_2}{\sqrt{2}}\right)^{m-n}L^{(m-n)}_{n}\left[\frac{\xi_1^2+\xi_2^2}{2}\right]
\end{split}\end{equation}
where $L^{(i)}_{j}[x]$ are associated Laguerre polynomials.

We can thus write the matrix element $\rho_{a,b,c,d}=\langle a,b|\rho|c,d\rangle$

\begin{equation}
\begin{split}
\rho_{a,b,c,d}=&\frac{1}{(2\pi)^2}\left(\frac{c!d!}{ a!b!}\right)^{\frac{1}{2}}\int d^{4}\xi\exp\left[-\frac{1}{4} \vekk{\xi}^T\Sigma (\Gamma+\iden) \Sigma^T \vekk{\xi}\right]
\left(\frac{\xi_1+i\xi_2}{\sqrt{2}}\right)^{a-c}\\&\left(\frac{\xi_3+i\xi_4}{\sqrt{2}}\right)^{b-d}L^{(a-c)}_{c}\left[\frac{\xi_1^2+\xi_2^2}{2}\right]L^{(b-d)}_{d}\left[\frac{\xi_3^2+\xi_4^2}{2}\right]
 \ .
\end{split}
\end{equation}

We first note that all matrix elements $\rho_{a,b,c,d}$, where $(a-c)+(a-d)$ is odd (or equivalently $(a+b+c+d)$ is odd) must vanish as the integrand is then an odd functions. The element $\rho_{0,0,0,0}$ may be found by Gaussian integration,
\begin{equation}
\rho_{0,0,0,0}=\frac{1}{(2\pi)^2}\int d^4\xi \exp\left[-\frac{1}{4} \vekk{\xi}^T\Sigma (\Gamma+\iden) \Sigma^T \vekk{\xi}\right]
\end{equation}

The integral converges if $\Gamma+\iden$ is positive, and  by recognising that the integral is invariant under symplectic transformations of $\Gamma+\iden$, in particular symplectic diagonalisation, one can reduce it to a product of standard Gaussian integrals to give,
\begin{equation}
\rho_{0,0,0,0}=\frac{4}{\gamma_1\gamma_1}=\frac{4}{|\Gamma+\iden|^\frac{1}{2}}
\end{equation}
where $\gamma_1$ and  $\gamma_2$ are symplectic eigenvalues of $\Gamma+\iden$ and $|\Gamma+\iden|$ is its determinant. We have used here the fact that the determinant of a matrix is invariant under symplectic operations.
To calculate the remaining matrix elements, 
we multiply out the multinomials in the expression and integrating each individually. Using the identity
\begin{equation}
x^ke^{-ax^2}=\left.\frac{\partial^k }{\partial j^k}e^{-ax^2+jx}\right|_{j=0}
\end{equation}
each term can be re-written as a differential.
%
We use the following identity to ``complete the square''
\begin{equation}%\begin{split}
-\frac{1}{4}\vekk{\xi}^T\Sigma(\Gamma+\iden)\Sigma^T\vekk{\xi}+\vek{j}^T\vekk{\xi}=-\frac{1}{4}\vekk{\xi}'^T\Sigma(\Gamma+\iden)\Sigma^T\vekk{\xi}'+\vek{j}^T\Sigma(\Gamma+\iden)^{-1}\Sigma^T\vek{j}
%\end{split}
\end{equation}
where $\vekk{\xi}'=(\vekk{\xi}-2\Sigma(\Gamma+\iden)^{-1}\Sigma^T\vek{j})$
and thus each multinomial term takes the following form,
\begin{equation}
\begin{split}
&\frac{1}{(2\pi)^2}\int d^4\xi \exp[-\frac{1}{4}\vekk{\xi}^T\Sigma(\Gamma+\iden)\Sigma^T\vekk{\xi}]\xi_1^{k_1}\xi_2^{k_2}\xi_3^{k_3}\xi_4^{k_4}\\&=\left[\frac{\partial^{k_1}}{\partial j_1^{k_1}}\frac{\partial^{k_2}}{\partial j_2^{k_2}}\frac{\partial^{k_3}}{\partial j_3^{k_3}}\frac{\partial^{k_4}}{\partial j_4^{k_4}}\right]\int d^4\xi
\exp[-\frac{1}{4}\vekk{\xi}^T\Sigma(\Gamma+\iden)\Sigma^T\vekk{\xi}+\vek{j}^T\vekk{\xi}]\\
&=\frac{4}{|\Gamma+\iden|^{\frac{1}{2}}}\left[\frac{\partial^{k_1}}{\partial j_1^{k_1}}\frac{\partial^{k_2}}{\partial j_2^{k_2}}\frac{\partial^{k_3}}{\partial j_3^{k_3}}\frac{\partial^{k_4}}{\partial j_4^{k_4}}\right]\exp[\vek{j}^T\Sigma(\Gamma+\iden)^{-1}\Sigma^T\vek{j}]
\end{split}
\end{equation}

 Each matrix element can now be calculated by expanding its multinomials and differentiating as appropriate. Introducing, for convenience the matrix $B=(\Gamma+\iden)^{-1}$, we find that
\begin{eqnarray}
        \sigma_{1,0,1,0}&=&1-B_{1,1}-B_{2,2}, \nonumber\\
        \sigma_{0,1,0,1}&=& 1-B_{3,3}- B_{4,4}, \nonumber\\
        \sigma_{1,0,0,1}&=& - B_{1,3} - B_{2,4} + i(B_{1,4}- B_{2,3}), \nonumber\\
        \sigma_{2,0,0,0}&=& 2^{-1/2} (-B_{1,1} +B_{2,2}-2 i B_{1,2}), \nonumber\\
        \sigma_{0,2,0,0}&=& 2^{-1/2} (-B_{3,3} + B_{4,4} - 2 i B_{3,4}), \nonumber\\
        \sigma_{1,1,0,0}&=& -B_{1,3} + B_{2,4}-
        i(B_{1,4}+B_{2,3}).\label{en}
\end{eqnarray}
where $\sigma_{a,b,c,d}=\rho_{a,b,c,d}/\rho_{0,0,0,0}$.


Our analysis is now almost complete. We showed above that the most general states which are invariant under an iteration of the Gaussification protocol have null matrix elements $\rho_{a,b,c,d}$  when $(a+b+c+d)$ and are completely specified by ten free parameters, corresponding to the six matrix elements highlighted. We now see that for any choice of these parameters there exists a ``state'' with a Gaussian covariance matrix $\Gamma=B^{-1}-\iden$ (although it may not be a physical state satisfying the condition $\Gamma\ge -i\Sigma$), as long as $B^{-1}$ exists and is positive. This is the case as long as $|B|\neq0$. However, if we recall that $\rho_{0,0,0,0}=4|B|^{1/2}$, we see that $|B|$ is only zero when $\rho_{0,0,0,0}$ is zero, which is only the case when $\rho^{(\infty)}$ is the unphysical null state, so we can discount this.
Thus we have shown that the only states invariant under an iteration of the protocol  are Gaussian states with zero displacement. 

We now consider the criteria for convergence. First we ask, given a particular starting state to what state will it converge? Labelling the matrix elements of the starting state $\rho^{(0)}_{a,b,c,d}$ and choosing a normalisation such that $\rho^{(0)}_{0,0,0,0}=1$, we find from equation~(\ref{eq:recursion}) that the six matrix elements highlighted above converge to their final value after a single iteration, that is,
\begin{eqnarray}
        \rho^{(i)}_{1,0,1,0}&=&\rho^{(1)}_{1,0,1,0}=\rho^{(0)}_{1,0,1,0}-|\rho^{(0)}_{1,0,0,0}|^2 \nonumber\\
        \rho^{(i)}_{0,1,0,1}&=&\rho^{(1)}_{0,1,0,1} = \rho^{(0)}_{0,1,0,1} -|\rho^{(0)}_{0,1,0,0}|^2\nonumber\\
        \rho^{(i)}_{1,0,0,1}&=& \rho^{(1)}_{1,0,0,1}= \rho^{(0)}_{1,0,0,1} -\rho^{(0)}_{1,0,0,0}\rho^{(0)}_{0,0,0,1}\nonumber\\
        \rho^{(i)}_{2,0,0,0}&=&  \rho^{(1)}_{2,0,0,0}= \rho^{(0)}_{2,0,0,0}-(1/\sqrt{2})(\rho^{(0)}_{1,0,0,0})^2 \nonumber\\
        \rho^{(i)}_{0,2,0,0}&=& \rho^{(1)}_{0,2,0,0}=\rho^{(0)}_{0,2,0,0}-(1/\sqrt{2})(\rho^{(0)}_{0,1,0,0})^2 
 \nonumber\\
        \rho^{(i)}_{1,1,0,0}&=& \rho^{(1)}_{1,1,0,0}=\rho^{(0)}_{1,1,0,0}-\rho^{(0)}_{1,0,0,0}\rho^{(0)}_{0,1,0,0}
    \ .\label{firstiter}
\end{eqnarray}


One can show by induction in an analogous way as above for the simple pure state case that the states converge matrix-elementwise after many iterations to the Gaussian state with covariance matrix $B^{-1}-\iden$ where $B$ is calculated from the matrix elements of $\rho^{(1)}$ via the inverse of the relations in equations~(\ref{en}). Although the matrix elements always converge to their respective final values, the state as a whole can only converge if $B^{-1}-\iden$ corresponds to a physical covariance matrix, that is $B^{-1}-\iden\ge -i\Sigma$.

Thus we have proved all the assertions made at the start of this section. Namely that the only states invariant under the protocol are Gaussian states centred in phase space and that for any given starting supply $\rho^{(0)}$,  whether or not, and to which state it will converge  can be calculated analytically from just a small number of matrix elements of $\rho^{(0)}$.

\section{Examples}

\subsection{An example mixed input}
In chapter~\ref{ch:7}, we considered the states generated by a simple optical Procrustean entanglement concentration protocol. In particular we considered the states by generated  when the input state was a two-mode squeezed state where both modes had passed through absorbing channels with the same transmission coefficient $\tau$. In the limit that the initial squeezing was small, this process generates a family of entangled mixed states described by two real parameters $\lambda$, which can be take any real value between -1 and 1, by setting the beam splitter transmittivity in the Procrustean protocol to an appropriate value, and $\tau$ with the following matrix elements

\begin{equation}\label{mixedinputrhost}
\rho_{0,0,0,0}=\frac{1}{1+\lambda^2+\epsilon\lambda^2}
\end{equation}
\begin{equation}
\rho_{1,1,0,0}=\rho_{0,0,1,1}=\lambda\rho_{0,0,0,0}
\end{equation}
\begin{equation}
\rho_{1,1,1,1}=\lambda^2\rho_{0,0,0,0}
\end{equation}
\begin{equation}\label{mixedinputrhofin}
\rho_{0,1,0,1}=\frac{1-\tau}{\tau}\lambda^2\rho_{0,0,0,0}\ .
\end{equation}

Let us investigate how such a state is transformed by iterations of the Gaussification protocol. Firstly, by applying the procedure describe in section~\ref{sec:geninput} we calculate the covariance matrix $\Gamma$ of the Gaussian state to which the state elementwise converges

\begin{equation}
\Gamma=\frac{1}{\tau-\lambda^2}\left(\begin{array}{cccc}\tau+\lambda^2(2\tau-1)&0&2\lambda\tau&0\\
0&\tau+\lambda^2(2\tau-1)&0&-2\lambda\tau\\
2\lambda\tau&0&\lambda^2+\tau&0\\
0&-2\lambda\tau&0&\lambda^2+\tau
\end{array}
\right)
\end{equation}

This covariance matrix only corresponds to a physical state fulfilling $\Gamma+i\Sigma\ge0$ if the condition $\tau>\lambda^2$ is met, thus statewise convergence can only occur when this is fulfilled. In figure~\ref{fig:t50ent} we plot, as a function of $\lambda$, the logarithmic negativity, $\tau=0.5$ of the input state, the state generated by one and two iterations of the protocol and the limiting state to which the protocol is converging. We see a marked increase in the entanglement after each iteration, in spite of the fact that the input states is not pure. The entropy of these states is depicted in figure~\ref{fig:t50entropy}. We see that the entropy of the final state is, in fact, higher than the starting state, and the entropy increases with each iteration accordingly. In figure~\ref{fig:t50prob} we see the success probability for each iteration. In particular this probability is greater than 50\% for most values of $\lambda$ below the convergence threshold. Comparing this plot to figure~\ref{fig:pureprob} indicates that the success probability is little affected by the mixedness of the input state.



The simultaneous increase in  both the entanglement and the von Neumann entropy of the state increase. This is in marked contrast to entanglement distillation protocols for qubits, where an increase in entanglement is usually accompanied by a decrease in entropy, since for any given degree of entropy of the state there is a maximum amount of entanglement which the system may possess \cite{frankandkoenmems,munromems}. This is also true for Gaussian states \cite{italiangaussmems}, although not for  infinite dimensional states in general, but for a given entropy the maximally allowed entanglement is much larger \cite{italiangaussmems}. This explains the seemingly counter-intuitive behaviour seen here. Of course, for application of entangled states  to quantum key distribution, for the highest security and key rate, pure entangled states are desirable. In the next example we investigate the criteria for the convergence of the protocol towards a pure state, and give an example to illustrate this.


\begin{figure}
\psfrag{en}{\large $E_\mathcal{N}$}
\psfrag{lam}{\large $\lambda$}
\begin{center}
\includegraphics{t50ent.eps}
\end{center}
\caption{\label{fig:t50ent}This figure depicts the logarithmic negativity $E_\mathcal{N}$ as a function of $\lambda$ for, i) the initial state $\rho$ specified in equations~(\ref{mixedinputrhost}) to~(\ref{mixedinputrhofin}) where we set $\tau=0.5$  ii) the state generated by a single (dashed) and two iterations (wider dashing) of the protocol and iii) the limiting state (solid line). Note that the limiting value only exists for values of $\lambda<\sqrt{\tau}$, since above this value the protocol does not converge.}
\end{figure}
\begin{figure}
\psfrag{S}{\large $S_\textrm{vN}$}
\psfrag{lam}{\large $\lambda$}
\begin{center}
\includegraphics{t50entropy.eps}
\end{center}
\caption{\label{fig:t50entropy} Here we plot the von Neumann entropy $S_\textrm{vN}$ for the initial (dotted), first (dashed) and second (wider dashing) iterations and the limiting state (solid line) for the input state $\rho$ specified in equations~(\ref{mixedinputrhost}) to~(\ref{mixedinputrhofin}). We see that the entropy of the limiting state is non-zero and this is reflected in entropy increases at each iteration.}
\end{figure}

\begin{figure}
\psfrag{pr}{\large $P$}
\psfrag{lam}{\large $\lambda$}
\begin{center}
\includegraphics{t50prob.eps}
\end{center}
\caption{\label{fig:t50prob} Here we see the success probability $P$ for the first (dashed) and second (wider dashing) iterations of the protocol with input supply  $\rho$ specified in equations~(\ref{mixedinputrhost}) to~(\ref{mixedinputrhofin}).}
\end{figure}



\subsection{Convergence to a Pure State}

It is a straightforward consequence of the results in section~\ref{sec:geninput} that certain mixed input state supplies will converge to a pure Gaussian state. Since any pure two-mode centred Gaussian state $\rho$ may be written $\hat{O}\hat{S}_1(\zeta_1)\hat{S}_2(\zeta_2)\ket{0,0}$ where $\hat{O}$ is a general passive linear two-mode transformation and $\hat{S}_i(\zeta_i)$ is a single mode squeezing operation \cite{wolfentpower}, since the squeezing operators are quadratic in annihilation and creation operators, matrix elements $\rho_{1,0,1,0}$, $\rho_{0,1,0,1}$ and $\rho_{1,0,0,1}$ are zero. Using the map between these matrix elements and the covariance matrix $\Gamma$ introduced in section~\ref{sec:geninput} we can verify that these conditions alone suffice to ensure that $\Gamma$ has unit determinant. Thus these matrix elements being zero is a  necessary and sufficient condition  ensure that $\rho$ is pure.

Equations~(\ref{firstiter}) and this condition leads directly to the following conditions on the input supply for convergence to a pure Gaussian state,

\begin{equation}\begin{split}
&\rho_{1,0,1,0}^{(0)}=|\rho_{1,0,0,0}^{(0)}|^2/\rho_{0,0,0,0}^{(0)}\\
&\rho_{0,1,0,1}^{(0)}=|\rho_{0,1,0,0}^{(0)}|^2/\rho_{0,0,0,0}^{(0)}\\
&\rho_{1,0,0,1}^{(0)}=\rho_{1,0,0,0}^{(0)}\rho_{0,0,0,1}^{(0)}/\rho_{0,0,0,0}^{(0)}
\end{split}
\end{equation}
provided $\rho_{0,0,0,0}$ and the conditions of convergence described in section~\ref{sec:geninput} are fulfilled.

Let us consider an simple example of a mixed input state which fulfils these criteria.
\begin{eqnarray}
    \rho_{0,0,0,0}&=&1/(1+\varepsilon^2),
    \,\,
    \rho_{1,1,0,0} =\rho_{0,0,1,1} = \varepsilon/(2+2\varepsilon^2)\nonumber\\
     \rho_{1,1,1,1}&=&\varepsilon^2/(1+\varepsilon^2)\label{topure}
\end{eqnarray}
with $\varepsilon\in [0,1)$, and $\rho_{a,b,c,d}=0$ otherwise.

The limiting state, to which repeated iterations of the protocol on this input will tend, is a pure two-mode squeezed state with squeezing $\tanh(r)=-\varepsilon/2$. How the  degree of entanglement and entropy evolves under repeated iteration of the protocol on this state  are plotted in figures~\ref{fig:topureent} and~\ref{fig:topureentropy}. Although for more highly mixed states the entropy increases after the first iteration, we see that after repeated iterations the entropy decreases for all values of $\varepsilon$, as it tends to zero.

\begin{figure}
\psfrag{en}{\large $E_\mathcal{N}$}
\psfrag{lam}{\large $\varepsilon$}
\begin{center}
\includegraphics[width=10cm]{topureent.eps}
\end{center}
\caption{\label{fig:topureent}This figure plots the logarithmic negativity $E_\mathcal{N}$ as a function of $\varepsilon$ for, i) the initial state $\rho$ specified in equation~(\ref{topure})  ii) the state generated by a single (dashed) and two (wider dashing) iterations  iii) the limiting pure two-mode squeezed state (solid line).}
\end{figure}
\begin{figure}
\psfrag{S}{\large $S_\textrm{vN}$}
\psfrag{lam}{\large $\varepsilon$}
\begin{center}
\includegraphics[width=10cm]{topure.eps}
\end{center}
\caption{\label{fig:topureentropy} Here we plot the von Neumann entropy $S_\textrm{vN}$ for the initial (dotted), first (dashed) and second (wider dashing) and fourth (widest dashing) iterations of the protocol on state $\rho$ described in equation~(\ref{topure}). The limiting state is a pure two-mode squeezed state, the entropy of which vanished.}
\end{figure}

Thus we have demonstrated that, under ideal experimental conditions, a Procrustean protocol with a non-Gaussian element, such as the one introduced in the last chapter, can be combined with this Gaussification, to give a scheme which can distill Gaussian states of higher entanglement, and for certain input states, of lower entropy. 
This is the first, and so far only, entanglement distillation procedure based on realistic operations to be proposed for continuous variable states. 
We focussed here on entanglement distillation, but a simplification of the protocol to one site only, also leads to a scheme for the   generating single-mode squeezed pulses with a far greater squeezing than can be generated via current non-linear techniques.
In the next chapter, we shall continue our analysis of the Gaussification protocol by considering how well it might perform under the imperfect operations which would be implemented in a real laboratory.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "C:\\Documents and Settings\\dan\\My Documents\\Thesis\\Chapters\\thesis"
%%% TeX-master: "C:\\Documents and Settings\\dan\\My Documents\\Thesis\\Chapters\\thesis"
%%% End: 


==> c7new.tex <==
%auto-ignore
\chapter{Distillation of continuous variable entanglement}\label{ch:7}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Distribution of Entanglement}\label{sec:entdistrib}

As discussed in section~\ref{ch:1}, many of the most intriging features and useful applications of entanglement are encountered when the entangled sub-systems are spatially separated. Entangled states, however, can only be created by global operations on the sub-systems, which requires either that the sub-systems interact directly with one another, or each intereacts directly with some  mediating third party , as in the protocols described in chapters~\ref{ch:4} and~\ref{c-5}. In either case, for entanglement to be established between two distant laboratories, quantum systems must physically traverse  the distance between them.

It is unavoidable that during this tranmission, some interaction with the ``envirnoment'', which is how we shall describe systems outside of the experimenter's control, will occur. This usually leads to the state of the system changing,  typically becoming  more mixed due to entanglement with the environment. This in turn, degrades the entangled state which is supposed to be being transmitted.

As an example of this, let consider a two-mode squeezed state, as introduced in section~\ref{sec:gausstates}, with real squeezing parameter $\lambda$, generated at a central source of pulsed radiation. The two pulses are transmitted separately through  optical fibres channels  to two parties, who we shall name Alice and Bob\footnote{The use of the names Alice and Bob, instead of the dry labelling  $A$ and $B$, has been adopted from classical communication theory to become ubiquitous in quantum information science. Indeed, it is hard to find a paper on quantum key distribution or entanglement distillation where they do not appear!}.

To a first approximation, an optical fibre acts as an \emph{absorbing channel}.This is a transmission line  which absorbs some of the radiation which passes through it. A thorough analysis \cite{stefanchannelpaper} has shown that such a channel may be accurately modelled in a very simple way. We pretend that the light pulse has been mixed with a vacuum mode on a beam splitter of transmittivity $T=\sqrt{\tau}$. The parameter $\tau$ then corresponds to the \emph{transmission coefficient} of the channel, expressing the ratio between the intensities of transmitted and incident light. Since the beam splitter is a Gaussian operation, the absorbing channel preserves the Gaussian nature of input states. %For this reason, it is often called a Gaussian channel.
%
In the phase-space formalism it is easy to calculate the effect of such a channel. The displacement vector is reduced by a factor of $\sqrt{\tau}$, and the covariance matrix $\Gamma$ transforms to $\tau \Gamma +(1-\tau)\iden$.

Let us consider the effect of passing both pulses of a two-mode squeezed state with real squeezing parameter $r$ through two channels, each with equal transmission coefficients. The covariance matrix is transformed, from the form expressed in equation~(\ref{eq:tmss}) to

\begin{equation}\label{eq:noisytmss}
\left(\begin{array}{cccc}
1+\tau(C_r-1) &0&- \tau S_r&0\\
0&1+\tau(C_r-1) &0& \tau S_r\\
-\tau S_r&0&1+\tau(C_r-1) &0\\
0&\tau S_r&0&1+\tau(C_r-1) 
\end{array}
\right)
\end{equation}
where $C_r=\cosh(2r)$ and $S_r=\sinh(2r)$ as before.
%
We can calculate the logarithmic negativity of this state using the method described in the previous section, and find,
%
\begin{equation}
E_\mathcal{N}=-\log_2[1-\tau(1-e^{-2r})]\ .
\end{equation}
Thus, as expected, while entanglement still increases with increasing $r$, the absorbtion $\tau<1$ reduces its value. Furthermore, while the entanglement of the pure two-mode squeezed state is unbounded, the entanglement of the state after the absorbing channels, is bounded by $-\log_2[1-\tau]$.

\section{Entanglement Distillation}\label{sec:distillsec}

In fact, this degradation in the entanglement of the states at their source is a generic feature of the decoherence processes which are unavoidable in the  transmission of quantum states. For the applications of spatially distributed entangled Gaussian states discussed above in section~\ref{sec:gausstates}, highly entangled states are required. Since, by definition, the entanglement of a spatially distributed state cannot be increased by local operations and classical communication, another approach is required. This problem was first considered for qubit systems, and  Bennett and co-workers proposed a scheme \cite{bennettdistillation} whereby if the two spatially separated parties, Alice and Bob, share a supply of many copies of a mixed and weakly entangled state, which had a fidelity greater than $1/2$ with respect to a maximally entangled state, they could
 by two-qubit operations, measurement and classical communication \emph{distill} a small number of copies of states arbitrarily close to a maximally entangled state. 

Clearly, the quantum systems most appropriate for transmission over long distances are light pulses. Light pulses can embody qubits in, for example, their polarisation, and schemes for the implementation of the quantum gates needed for entanglement distillation have been proposed \cite{klm}. However, these schemes are very technically challenging and in particular, a full scheme would required detectors with close to unit efficiency, which are so far unavailable. So far, therefore, only a few steps of such a scheme have been implemented \cite{pandistillation}. 

Of course, light pulses can also distribute entangled Gaussian states, which we have seen in the previous chapter, have many applications in quantum information science. It is thus natural to ask whether one can distill Gaussian states. In particular, since Gaussian operations are so experimentally accessible, it would be ideal to have an entanglement distillation protocol for Gaussian states which employed solely these operations.




\section{Distillation with Gaussian operations}

With the formal description of Gaussian operations, which we have outlined above, the question of finding a Gaussian entanglement distillation procedure becomes an matter of matrix analysis. This  was carried out in \cite{impnogauss}, \cite{jaromirnogauss} and \cite{giedkenogauss}. Their proofs are too technical to sketch here, but, in light of what \emph{is} possible with Gaussian operation s alone, the result is surprising. If one acts with solely Gaussian operations and measurements on a supply of Gaussian states it is impossible to distill any greater entanglement than the initial states already possess. Any joint operations, measurements and classical communication which Alice and Bob implement will leave them with a state with either the same or less entanglement than in the initial states\footnote{A corollary of their result, due to the correspondance between entanglement distillation schemes and quantum error correction \cite{bennettcorrespondance}, is that no quantum error correction scheme based on Gaussian operations can correct Gaussian errors on Gaussian states. This is surprising in light of \cite{braunsteinerrorcorlinop} which showed that arbitrary errors with a \emph{discrete} probability distribution may be corrected with linear optics and homodyne detection. However, \cite{impnogauss,jaromirnogauss,giedkenogauss} implies that even the tiniest Gaussian error cannot be corrected by linear optics alone\cite{giedkepriv}.}.

This seems a disappointing result, but there is a loophole, that means that optical distillation of Gaussian states is not entirely ruled out. There is one operation avaliable to the linear optics lab, which is not a Gaussian operation. This is photo-detection. In the next section, we will show that even very simple protocols using passive linear optics and photo-detection can allow Alice and Bob to generate states more highly entangled than their initial supply, but the states will no longer be Gaussian.


\section{Procrustean Entanglement Enhancement with linear optics and photo-detection}\label{sec:procmeth}

\begin{figure}
\vspace{1cm}
\begin{center}
\includegraphics[width=10cm]{proc}
\end{center}
\caption{\label{fig:proc1} A ``Procrustean'' linear optical entanglement enhancement protocol. Bob mixes his half of a two-mode squeezed state with a single photon on a beam-splitter of transmittivity $T$ and places a photon counter at one of its output ports. }
\end{figure}
Imagine Alice and Bob share a pure two-mode squeezed state with real squeezing paramter $r$ and Bob performs the following operation. He mixes his entangled pulse with a single photon on a beam splitter with transmittivity $T$ as illustrated in figure~\ref{fig:proc1}, and measures, with a photo-detector one of the beam splitter outputs. Let us assume for now that the photo-detector works with 100\% efficiency and can resolve any number of photons in the measured mode. It is then a matter of algebra to show that after the measurement, if $m$ photons are registered Alice and Bob's state is collapsed into the following,


\begin{equation}
\ket{\psi}=\sqrt{\frac{1}{\sum_{n=m-1}^\infty|\alpha_n(m)|^2}}\sum_{n=m-1}^\infty \alpha_n \ket{n}_A\ket{n+1-m}
\end{equation}
where
\begin{equation}
\alpha_n(m)=(-\tanh(r))^n T^{n-m}R^{m-1}\left[-R^2\sqrt{{n \choose m}(n+1-m)}+T^2\sqrt{{n \choose m-1}m}\right]
\end{equation}
and we have assumed for simplicity that $T$ and $R$ are real, and we define ${n \choose k}=0$ if $k>n$.

As this is a pure state, one can immediately calculate the entanglement shared by Alice and Bob in terms of teh von Neumann entropy of the reduced density matrix $\rho_A$, $E_{vN}=-\textrm{Tr}[\rho_A \log_2 \rho_A]$. The analytic form of this does not give us much insight, so we shall plot the entanglement of the state generated when $m$ photons are detected, and the probability that this will occur (given a perfect detector) in figure~\ref{fig:procrus1}

\begin{figure}
\includegraphics[width=14cm]{procfig}
\caption{\label{fig:procrus1}The pure state entanglement (a) of the state generated and  probability (b) of the event, when a certain photon-number is detected in the simple protocol described in section~\ref{procmeth}, on a initial two-mode squeezed state with squeezing parameter $\tanh(r)=0.1$, shared by Alice and Bob, when a beam-splitter of transmittity $T=\tanh(r)=0.1$ is used. The probabilities which are close to zero and can thus not be read clearly on the graph decrease exponentially, e.g. for 2-photons the probability is $3\times10^{-4}$ and for 3-photons the probability is $4\times10^{-6}$. For comparison, the pure state entanglement of the input state is $0.08$.}
\end{figure}

This shows that with this very simple protocol employing the non-Gaussian operation of photo-detection, a huge gain in entanglement is acheivable, if at a very low probaility. 
The effect of the beam-splitter and the photo-detector is to single out a particular  decomposition of the input state, of which the part corresponding to zero-photons in the detector has a high amplitude and  very weakly entanglement, and the 1-photon part has low amplitude and high entanglement. %Such ``brute-force'' methods of increasing the entanglement of a state probabilistically are called Procrustaen {\bf i think i cite charlie bennett here!} after the {\bf talk about procustes and his leg chopping}
For the low values of $r$ which are expermeintally attainable, the probability of a two-or-more photon detection event is low, however, the beamplitter parameters can alsways be chosen such that, as in figure~\ref{fig:procrus1} the one-photon detection event corresponds to the most highly entangled state.

The fact that an entanglement of almost 1 is obtained in the above example is not accidental, since the value of $T$ was been chosen to ensure this. If one chooses $T\approx \tanh(r)/\lambda$ for some value $\lambda$, then the state generated conditional on one photon being detected is approximately $\ket{0}\ket{0}-\lambda\ket{1}\ket{1}$, the approximation being more and more valid as the original squeezing $r$ decreases. Thus the above method generates approximate Bell states, conditionaly on a particular measurement outcome being obtained. In the next section we shall see an important and relevant use for such states.

So far we have assumed perfect conditions, which we shall now relax. Firstly, we have assumed that the detector is both 100\% efficient and resolves different photon numbers. However, since the probability of 2-or-more photon detection event occurring is so small, when the detector does click it can be assumed that only 1 photon was present, thus the use of an inefficient detector which merely registers the presence or absence of photons will only minimally affect the state produced, leading to a tiny admixture of the states from these multi-photon detection events. 

Secondly, if Alice also possesses such a photo-detector, Bob does not need a single-photon sources, which are a great technological challenge. If the pair is willing to sacrifice some entangled pairs, Bob need only wait till Alice detects a single photon on her side of a pair and this will project Bob's counterpart into a single photon which he can use.

Most importantly, if the protocol were realised between distant laboratories, the light pulses will have passed to Alice and Bob via a channel which will at the very least absorb some of the signal decreasing the entanglement and increasing the entropy of the initial state avaliable to Alice and Bob. Thus it is natural to ask whether this protocol can give a similar boost in entanglement for  a mixed input state. We consider here the state described by covariance matrix in equation~(\ref{eq:noisytmss}). The matrix elements of the state generated yb the Procustean protocol, in the case when one and only one photon is incident on the detector may be calculated analytically, and the entanglement of the state, in terms of its logarithmic negativity thus calculated. We plot, in figure~\ref{noisyproc} the entanglement of the state before and after a successful implementation of the protocol. We see that even for these mixed states, this extremely simple procedure can provide a significant increase in the entanglement.

It will be convenient for the next chapter to write out the zero-photon and one-photon matrix elements of the (unnormalised) state $\rho$ generated here.
\begin{equation}
\rho_{0,0,0,0}=1
\end{equation}
can be set for convenience since $\rho_{0,0,0,0}>0$.
\begin{equation}
\rho_{1,1,0,0}=\rho_{0,0,1,1}=\lambda\rho_{0,0,0,0}
\end{equation}
\begin{equation}
\rho_{1,1,1,1}=\lambda^2\rho_{0,0,0,0}\left(1+(\tau-1)\tanh^2(r)\right)
\end{equation}
\begin{equation}
\rho_{0,1,0,1}=\epsilon\lambda^2\rho_{0,0,0,0}\left(1-(\tau-1)\tanh^2(r)\right)
\end{equation}
where 
\begin{equation}
\lambda=\frac{(2T^2-1)\tanh(r)\tau}{T(\tanh^2(r)(\tau-1)^2)-1}
\end{equation}
and $\epsilon=(1-\tau)/\tau$. All other zero and one photon matrix elements are zero.
%
%
Note that when $r$ is very small, these matrix elements depend only on the two parameters $\epsilon$ and $\lambda$, and furthermore for any given values of $r$ and $\tau$, $\lambda$ may be set by choosing the appropriate value of $T$.

\begin{figure}
\includegraphics[width=15cm]{noisyplots}
\caption{\label{noisyproc} In this figure we see the result of the procrustean entanglement concentration  protocol on a mixed input state which is the result of a two-mode squeezed state with squeezing $\tanh(r)=0.1$  being passed through absorbing channels with transmission coefficient $\tau$. The beam splitter transmittivity is chosen to be $T=0.1$,  the same as the plot in figure~\ref{fig:procrus1}. In plot (a) the entanglment of the generated state is plotted alongside the entanglement of the input state (dotted line) as a function of $\tau$. In plot (b) we see that teh success probability has decreases weakly and linearly with decreasing $\tau$.}
\end{figure}


The first investigation of local measurement-base protocols for probabilistically increasing the entanglement of a state can be found in \cite{bennettprocust} who coined the term ``Procrustean'' for simple measurement-based protocols on a single copy of the state\footnote{Procrustes was a villain in Greek legend, who would invite travellers to sleep in his iron bed, promising that it would be a perfect size for them. However, this perfect fit was achieved by  shorter guests being stretched or chopping off the legs of taller ones! The entanglement concentration methods here are Procustean, in the sense that the projection, corresponding to the successful measurement outcome, ``chops off'' the more weakly entangled portion of the state leaving a more highly entangled state behind.}.
The protocols described here were introduced by us in \cite{brownegauss} and \cite{jensgauss}, but a more comprehensive investigation of similar ideas can be found in \cite{billproc1,billproc2}. %Although, we have only considered a very simple non-Gaussian operation here, in fact a wide variety of non-linear operations can be implemented non-deterministically with passive linear optics, photon sources and measurement \cite{stefanmeasinduced}.
%
%
Since any kind of entanglement concentration or distillation is impossible with Gaussian operations, it is perhaps surprising how well these very simple Procrustean protocols with a single photo-detection as their only non-Gaussian element can enhance the entanglement of their input states, both pure and mixed.
Theses states however, are manifestly non-Gaussian. It would therefore appear, at first sight, that these protocols still do not aid us in the search for an entanglement distillation procedure for Gaussian states. In the next chapter, however, we introduce a simple linear optical protocol called ``Gaussification''. We will show that this allows Alice and Bob, via local linear optics operations, measurements and classical communication only, to convert entangled non-Gaussian states into Gaussian states and also, often, further increase the entanglement in the process.


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "C:\\Documents and Settings\\dan\\My Documents\\Thesis\\Chapters\\thesis"
%%% TeX-master: "C:\\Documents and Settings\\dan\\My Documents\\Thesis\\Chapters\\thesis"
%%% End: 


==> frontmatter.tex <==
%auto-ignore
%\chapter{Abstract}
\clearpage \pagestyle{empty}

%\clearpage \pagestyle{empty}
%\begin{center}
%  {\Huge Acknowledgements}\\[1cm]
%\end{center}
%To people

\begin{center}
  {\Huge Abstract}\\[1cm]
\end{center}


In this thesis, we introduce and evaluate several new procedures for the generation and manipulation of entangled states in quantum optical systems. Each scheme is evaluated in terms of realistic models of the imperfect apparatus of any real laboratory implementation. 

The first set of proposals concerns atoms interacting with optical cavities.
We describe a  method of generating maximally entangled states in the states of the electro-magnetic fields of two microwave cavities by the passage of an atom between them and its subsequent measurement. We demonstrate the natural robustness of this approach against a variety of experimental imperfections. 

We then introduce a further scheme for the generation of maximally entangled states between pairs atoms or ions trapped in  separate cavities. The ions are weakly driven by an external field and a leaking photon  from one cavity is  detected, after passing through a beam splitter to erase which-path information. In the ideal case, this leads to the deterministic generation of high fidelity states, and when more realistic conditions are assumed, still allows high fidelity states to be generated in a heralded non-deterministic manner.

In the final part of the thesis, we turn our attention to the manipulation of entangled states of light pulses. Entanglement distillation has many applications in quantum information science. 
Gaussian states are the natural states of light pulses produced in laser experiments, and  standard optical operations preserve the Gaussian form.
 Entanglement distillation on Gaussian states is impossible with these operations alone. We illustrate that the additional element of photon detection enables one to circumvent this restriction, but produces highly non-Gaussian states. We then introduce a simple  protocol, which we call ``Gaussification'', which allows more highly entangled approximately Gaussian states to be distilled from a non-Gaussian supply. Together, these procedures form the first realistic entanglement distillation scheme for Gaussian states. We analyse fully the convergence characteristics of the protocol and assess the operation of the scheme with the imperfect operations one could expect in a real laboratory implementation.



\tableofcontents
%\listoffigures
%\listoftables

% Local Variables:
% TeX-master: "./thesis"
% End:



==> publications.tex <==
%auto-ignore
\chapter*{List of Publications}


%\vspace{3.5cm}
\begin{itemize}
\item \textbf{Resonance fluorescence in intense laser fields}.
\\
D.E. Browne and C.H. Keitel, 
 \textit{Journal of Modern Optics},
\textbf{47}, 1307 (2000).

\item \textbf{Measurement-based quantum computation on cluster states}. \\R. Raussendorf, D.E. Browne and H.J. Briegel, \textit{Physical Review A}, \textbf{68}, 022312 (2003).


\item \textbf{Symmetric qubits from cavity states}. \\ D.E. Browne and M. B. Plenio, \textit{Physical Review A}, \textbf{66}, 042307 (2003).

\item \textbf{Robust generation of entanglement between two cavities mediated by short interactions with an atom}. \\ D.E. Browne and M. B. Plenio, \textit{Physical Review A}, \textbf{67}, 012325 (2003).
(contains work used in chapter~\ref{ch:4})

\item \textbf{Robust creation of entanglement between ions in spatially separate cavities}. \\ D.E. Browne, M. B. Plenio and S.F. Huelga, \textit{Physical Review Letters}, \textbf{91}, 067901 (2003).
(contains work used in chapter~\ref{ch:5})


\item \textbf{Driving non-Gaussian to Gaussian states with linear optics}. \\ D.E. Browne, J. Eisert, S. Scheel and M. B. Plenio, \textit{Physical Review A}, \textbf{67}, 062320 (2003).
(contains work used in {\bf which chapter?})


\item \textbf{Distillation of continuous-variable entanglement with optical means}. \\ J. Eisert, D.E. Browne, S. Scheel and M. B. Plenio, \textit{Annals of Physics}, \textbf{311}, 431 (2004).
(contains work used in {\bf which chapter?})



\item \textbf{Resource Efficient Linear Optics Quantum Computation}. \\ D.E. Browne and T. Rudolph, e-print quant-ph/0405157, submitted for publication to  \textit{Physical Review Letters} {\bf I hope I will be able to update this!}
\end{itemize}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "C:\\Documents and Settings\\dan\\My Documents\\Thesis\\Chapters\\thesis"
%%% End: 


==> statement.tex <==
%auto-ignore
%\chapter*{Statement on collaborative work}

%The work reported in this thesis was the result of several fruitful collaborations. 
%The  entanglement generation proposal reported in chapter 4  was developed a collaboration with Martin Plenio, my supervisor. I initiated the project and played a leading role in its development, carrying out the majority of the analytical calculations.
%%
%The entanglement generation scheme described in the latter sections of chapter 5 was developed in collaboration with Martin Plenio and Susanna Huelga. I contributed part of the analytic calculations and numerical simulations for this project.
%%
%The work on the distillation of entangled Gaussian states described in chapters 7 and 8 was carried out with Jens Eisert, Stefan Scheel and Martin Plenio. I took a leading role in all stages of this work. I performed a large part of the analytic work and carried out most of the numerical simulations for the project, including all of those whose results appear in this thesis.

%\vspace{2cm}

%\textbf{Dan Browne},  17th December 2004


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "C:\\Documents and Settings\\dbrowne\\My Documents\\Thesis\\Chapters\\thesis"
%%% End: 

